Operator-Valued Q-Learning: Compositional Bellman Recursions for Order-Sensitive Decision Making

In quantum pulse sequences, spacecraft attitude control and in-hand reorientation, actions act on a hidden physical state as non-commuting operators, so the outcome of a plan depends on the order of its actions. We let the value function carry this structure: each Q(s,a) is an N x N operator, and the Bellman backup applies the action's dual map to the continuation value, Q(s,a) = K_a^*(R(s,a) + gamma E V(s')). Unrolled along a plan, the recursion builds the ordered product of the actions' operators, and the value at any latent state is a linear trace readout. It is exact for policies that do not observe the latent, the backup contracts for unitary and orthogonal dynamics, and an asynchronous operator TD scheme learns it with almost-sure convergence. Classical values live in a lattice, so a maximum over actions exists; self-adjoint operators form an anti-lattice (Kadison) and have none. An operator log-sum-exp still gives one operator per state-action pair whose readout upper-bounds the value of every policy at every latent state. The sampled update converges to it for a finite horizon, and it reduces to soft Q-learning and the QMDP bound when actions commute. We prove that scalar values on observations that ignore action order must confuse swapped histories, that exact history tables grow exponentially for free action groups but polynomially for nilpotent ones, and give a Hankel-rank lower bound on the operator dimension. In experiments the learned policy matches 1000-simulation tree search on SO(3) pointing for horizons up to 20 at ~10^4 times lower decision cost, transfers zero-shot to unseen initial states, and acts exactly on its belief mean when the initial state is hidden, where plugging the mean into a DQN does not. A planner with the same model knowledge is more sample-efficient at short horizons, and a DQN given the operators matches or exceeds OpQ.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/tab_2x2_fixed_full.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llcccccc@{}}
\toprule
 & & \multicolumn{2}{c}{C1 random OLDP} & \multicolumn{2}{c}{C2 SO(3) pointing} & \multicolumn{2}{c}{C3 two-qubit} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Agent & $K_a$ & 100 & 3000 & 100 & 3000 & 100 & 3000 \\
\midrule
DQN on $\rho_t$ (nonlinear) & unknown & $\mathbf{0.96}${\scriptsize$\pm$0.02} & $\mathbf{1.00}${\scriptsize$\pm$0.00} & $0.85${\scriptsize$\pm$0.06} & $\mathbf{0.98}${\scriptsize$\pm$0.01} & $-0.08${\scriptsize$\pm$0.16} & $\mathbf{1.00}${\scriptsize$\pm$0.00} \\
DQN + $K_a$ data (nonlinear) & known & $0.91${\scriptsize$\pm$0.08} & $\mathbf{1.00}${\scriptsize$\pm$0.00} & $0.81${\scriptsize$\pm$0.03} & $\mathbf{0.98}${\scriptsize$\pm$0.01} & $0.26${\scriptsize$\pm$0.33} & $\mathbf{1.00}${\scriptsize$\pm$0.00} \\
Linear-Q (linear) & unknown & $0.86${\scriptsize$\pm$0.08} & $0.99${\scriptsize$\pm$0.00} & $0.73${\scriptsize$\pm$0.06} & $0.95${\scriptsize$\pm$0.02} & $0.21${\scriptsize$\pm$0.14} & $0.28${\scriptsize$\pm$0.00} \\
OpQ-soft (linear) & known & $0.77${\scriptsize$\pm$0.06} & $0.84${\scriptsize$\pm$0.01} & $\mathbf{0.94}${\scriptsize$\pm$0.02} & $\mathbf{0.98}${\scriptsize$\pm$0.00} & $\mathbf{0.38}${\scriptsize$\pm$0.20} & $0.83${\scriptsize$\pm$0.08} \\
\midrule
Linear-Q, max backup & unknown & $0.86${\scriptsize$\pm$0.08} & $0.99${\scriptsize$\pm$0.00} & $0.75${\scriptsize$\pm$0.06} & $0.97${\scriptsize$\pm$0.00} & $0.28${\scriptsize$\pm$0.00} & $0.46${\scriptsize$\pm$0.27} \\
DQN, 4 updates & unknown & $0.92${\scriptsize$\pm$0.03} & $1.00${\scriptsize$\pm$0.00} & $0.79${\scriptsize$\pm$0.11} & $0.99${\scriptsize$\pm$0.01} & $0.17${\scriptsize$\pm$0.38} & $1.00${\scriptsize$\pm$0.00} \\
DQN + $K_a$ data, 4 updates & known & $0.96${\scriptsize$\pm$0.02} & $1.00${\scriptsize$\pm$0.00} & $0.93${\scriptsize$\pm$0.02} & $0.99${\scriptsize$\pm$0.00} & $0.36${\scriptsize$\pm$0.22} & $1.00${\scriptsize$\pm$0.00} \\
DQN + $K_a$ data, true $R$ & known & $0.96${\scriptsize$\pm$0.04} & $1.00${\scriptsize$\pm$0.00} & $0.84${\scriptsize$\pm$0.05} & $0.99${\scriptsize$\pm$0.01} & $0.24${\scriptsize$\pm$0.32} & $1.00${\scriptsize$\pm$0.00} \\
DQN + $K_a$ data, reachable $\rho$ & known & $0.96${\scriptsize$\pm$0.03} & $1.00${\scriptsize$\pm$0.00} & $0.88${\scriptsize$\pm$0.04} & $0.98${\scriptsize$\pm$0.01} & $0.27${\scriptsize$\pm$0.29} & $1.00${\scriptsize$\pm$0.00} \\
Model + exhaustive & known & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} \\
\bottomrule
\end{tabular}}
\caption{E19, all agents, fixed initial latent. Normalised return after 100 and 3000 episodes; mean $\pm$ s.d.\ over 5 seeds. Bold marks the best of the first four rows.}
\label{tab:e19-2x2-fixed}
\end{table}

==> tables/tab_2x2_random.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llcccccc@{}}
\toprule
 & & \multicolumn{2}{c}{C1 random OLDP} & \multicolumn{2}{c}{C2 SO(3) pointing} & \multicolumn{2}{c}{C3 two-qubit} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Agent & $K_a$ & 100 & 3000 & 100 & 3000 & 100 & 3000 \\
\midrule
DQN on $\rho_t$ (nonlinear) & unknown & $0.89${\scriptsize$\pm$0.03} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.73${\scriptsize$\pm$0.04} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.04${\scriptsize$\pm$0.12} & $\mathbf{0.87}${\scriptsize$\pm$0.02} \\
DQN + $K_a$ data (nonlinear) & known & $0.93${\scriptsize$\pm$0.03} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.82${\scriptsize$\pm$0.03} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.22${\scriptsize$\pm$0.15} & $0.86${\scriptsize$\pm$0.02} \\
Linear-Q (linear) & unknown & $0.77${\scriptsize$\pm$0.06} & $0.96${\scriptsize$\pm$0.02} & $0.57${\scriptsize$\pm$0.04} & $0.95${\scriptsize$\pm$0.01} & $0.25${\scriptsize$\pm$0.10} & $0.54${\scriptsize$\pm$0.08} \\
OpQ-soft (linear) & known & $\mathbf{0.95}${\scriptsize$\pm$0.01} & $0.95${\scriptsize$\pm$0.00} & $\mathbf{0.95}${\scriptsize$\pm$0.01} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $\mathbf{0.58}${\scriptsize$\pm$0.07} & $0.68${\scriptsize$\pm$0.00} \\
\midrule
DQN + $K_a$ data, 4 updates & known & $0.96${\scriptsize$\pm$0.02} & $1.00${\scriptsize$\pm$0.00} & $0.90${\scriptsize$\pm$0.03} & $1.00${\scriptsize$\pm$0.00} & $0.38${\scriptsize$\pm$0.09} & $0.90${\scriptsize$\pm$0.01} \\
Model + exhaustive & known & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} \\
\bottomrule
\end{tabular}}
\caption{E19, $2\times2$ comparison with random initial latents. Normalised return of the greedy policy (exact evaluation) after 100 and 3000 training episodes; mean $\pm$ s.d.\ over 5 seeds. The first four rows cross the form of the value function (linear or nonlinear in $\rho$) with knowledge of the operators $K_a$; bold marks the best of these four. The last three rows are controls: the linear class trained on $K_a$-generated transitions (the missing cell of the comparison), the same DQN with four gradient updates per environment step, and a planner that knows $K_a$, learns $R$ and $P$ from the same episodes and searches exhaustively.}
\label{tab:e19-2x2}
\end{table}

==> tables/tab_2x2_random_full.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llcccccc@{}}
\toprule
 & & \multicolumn{2}{c}{C1 random OLDP} & \multicolumn{2}{c}{C2 SO(3) pointing} & \multicolumn{2}{c}{C3 two-qubit} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Agent & $K_a$ & 100 & 3000 & 100 & 3000 & 100 & 3000 \\
\midrule
DQN on $\rho_t$ (nonlinear) & unknown & $0.89${\scriptsize$\pm$0.03} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.73${\scriptsize$\pm$0.04} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.04${\scriptsize$\pm$0.12} & $\mathbf{0.87}${\scriptsize$\pm$0.02} \\
DQN + $K_a$ data (nonlinear) & known & $0.93${\scriptsize$\pm$0.03} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.82${\scriptsize$\pm$0.03} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.22${\scriptsize$\pm$0.15} & $0.86${\scriptsize$\pm$0.02} \\
Linear-Q (linear) & unknown & $0.77${\scriptsize$\pm$0.06} & $0.96${\scriptsize$\pm$0.02} & $0.57${\scriptsize$\pm$0.04} & $0.95${\scriptsize$\pm$0.01} & $0.25${\scriptsize$\pm$0.10} & $0.54${\scriptsize$\pm$0.08} \\
OpQ-soft (linear) & known & $\mathbf{0.95}${\scriptsize$\pm$0.01} & $0.95${\scriptsize$\pm$0.00} & $\mathbf{0.95}${\scriptsize$\pm$0.01} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $\mathbf{0.58}${\scriptsize$\pm$0.07} & $0.68${\scriptsize$\pm$0.00} \\
\midrule
Linear-Q, max backup & unknown & $0.77${\scriptsize$\pm$0.05} & $0.97${\scriptsize$\pm$0.01} & $0.62${\scriptsize$\pm$0.04} & $0.96${\scriptsize$\pm$0.01} & $0.29${\scriptsize$\pm$0.07} & $0.53${\scriptsize$\pm$0.07} \\
DQN, 4 updates & unknown & $0.89${\scriptsize$\pm$0.04} & $0.99${\scriptsize$\pm$0.00} & $0.82${\scriptsize$\pm$0.04} & $0.99${\scriptsize$\pm$0.00} & $0.04${\scriptsize$\pm$0.11} & $0.87${\scriptsize$\pm$0.03} \\
DQN + $K_a$ data, 4 updates & known & $0.96${\scriptsize$\pm$0.02} & $1.00${\scriptsize$\pm$0.00} & $0.90${\scriptsize$\pm$0.03} & $1.00${\scriptsize$\pm$0.00} & $0.38${\scriptsize$\pm$0.09} & $0.90${\scriptsize$\pm$0.01} \\
DQN + $K_a$ data, true $R$ & known & $0.94${\scriptsize$\pm$0.02} & $0.99${\scriptsize$\pm$0.00} & $0.81${\scriptsize$\pm$0.01} & $0.99${\scriptsize$\pm$0.00} & $0.19${\scriptsize$\pm$0.14} & $0.89${\scriptsize$\pm$0.02} \\
DQN + $K_a$ data, reachable $\rho$ & known & $0.94${\scriptsize$\pm$0.02} & $1.00${\scriptsize$\pm$0.00} & $0.82${\scriptsize$\pm$0.04} & $0.99${\scriptsize$\pm$0.00} & $0.19${\scriptsize$\pm$0.14} & $0.87${\scriptsize$\pm$0.03} \\
Model + exhaustive & known & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} \\
\bottomrule
\end{tabular}}
\caption{E19, all agents, random initial latent. Normalised return after 100 and 3000 episodes; mean $\pm$ s.d.\ over 5 seeds. Bold marks the best of the first four rows.}
\label{tab:e19-2x2-random}
\end{table}

==> tables/tab_transfer.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
 & \multicolumn{2}{c}{C1} & \multicolumn{2}{c}{C2} & \multicolumn{2}{c}{C3} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Agent & train $\rho_0$ & held-out & train $\rho_0$ & held-out & train $\rho_0$ & held-out \\
\midrule
DQN on $\rho_t$ & $1.00${\scriptsize$\pm$0.00} & $0.86${\scriptsize$\pm$0.04} & $0.98${\scriptsize$\pm$0.01} & $0.96${\scriptsize$\pm$0.02} & $1.00${\scriptsize$\pm$0.00} & $0.46${\scriptsize$\pm$0.11} \\
DQN + $K_a$ data & $1.00${\scriptsize$\pm$0.00} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.98${\scriptsize$\pm$0.01} & $0.98${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $\mathbf{0.84}${\scriptsize$\pm$0.03} \\
DQN + $K_a$ data, reachable $\rho$ & $1.00${\scriptsize$\pm$0.00} & $0.88${\scriptsize$\pm$0.02} & $0.98${\scriptsize$\pm$0.01} & $0.96${\scriptsize$\pm$0.01} & $1.00${\scriptsize$\pm$0.00} & $0.59${\scriptsize$\pm$0.04} \\
Linear-Q & $0.99${\scriptsize$\pm$0.00} & $0.75${\scriptsize$\pm$0.03} & $0.95${\scriptsize$\pm$0.02} & $0.78${\scriptsize$\pm$0.02} & $0.28${\scriptsize$\pm$0.00} & $0.37${\scriptsize$\pm$0.05} \\
OpQ-soft & $0.84${\scriptsize$\pm$0.01} & $0.95${\scriptsize$\pm$0.00} & $0.98${\scriptsize$\pm$0.00} & $\mathbf{0.99}${\scriptsize$\pm$0.00} & $0.83${\scriptsize$\pm$0.08} & $0.68${\scriptsize$\pm$0.01} \\
\midrule
Model + exhaustive & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} & $1.00${\scriptsize$\pm$0.00} \\
\bottomrule
\end{tabular}}
\caption{E19, zero-shot transfer. Agents train for 3000 episodes at one fixed initial latent and are evaluated, without retraining, at that latent and on 8 held-out latents (normalised return, mean $\pm$ s.d.\ over 5 seeds). Bold marks the best held-out score among the first four agents of the $2\times2$ comparison.}
\label{tab:e19-transfer}
\end{table}
